Apodotiko: Enabling Efficient Serverless Federated Learning in Heterogeneous Environments

Federated Learning (FL) is an emerging machine learning paradigm that enables the collaborative training of a shared global model across distributed clients while keeping the data decentralized. Recent works on designing systems for efficient FL have shown that utilizing serverless computing technologies, particularly Function-as-a-Service (FaaS) for FL, can enhance resource efficiency, reduce training costs, and alleviate the complex infrastructure management burden on data holders. However, current serverless FL systems still suffer from the presence of stragglers, i.e., slow clients that impede the collaborative training process. While strategies aimed at mitigating stragglers in these systems have been proposed, they overlook the diverse hardware resource configurations among FL clients. To this end, we present Apodotiko, a novel asynchronous training strategy designed for serverless FL. Our strategy incorporates a scoring mechanism that evaluates each client's hardware capacity and dataset size to intelligently prioritize and select clients for each training round, thereby minimizing the effects of stragglers on system performance. We comprehensively evaluate Apodotiko across diverse datasets, considering a mix of CPU and GPU clients, and compare its performance against five other FL training strategies. Results from our experiments demonstrate that Apodotiko outperforms other FL training strategies, achieving an average speedup of 2.75x and a maximum speedup of 7.03x. Furthermore, our strategy significantly reduces cold starts by a factor of four on average, demonstrating suitability in serverless environments.

==> code/yaml_syntax_highlighting.tex <==
% Source: http://tex.stackexchange.com/questions/152829/how-can-i-highlight-yaml-code-in-a-pretty-way-with-listings




==> sections/05_fedlesscan.tex <==

\input{alg/server_client}

\subsection{Partitioning Clients}
\label{sec:tiers}
Our selection strategy separates reliable clients that do not miss their training rounds due to slow updates, timeouts, or failures from stragglers. Towards this, we partition the clients into three groups, i.e., (i) \textit{rookies}, (ii) \textit{participants}, and (iii) \textit{stragglers}. \textit{Rookies} are clients which have not participated in the FL training process and for which no behavioral data exists (\S\ref{sec:behavedata}). \textit{Participants} are the group of clients that can participate in the clustering process (\S\ref{sec:behavedata}, \S\ref{sec:ClientSelection}). In our strategy, we use clustering to group reliable clients with similar behavior together. Finally, \textit{stragglers} are clients that have missed one or more consecutive training rounds. They have the lowest priority in our selection process (\S\ref{sec:ClientSelection}) and are characterized by using a variable called \texttt{cooldown} as described in \S\ref{sec:behavedata}. Note that, our client selection strategy (\S\ref{sec:ClientSelection}) adapts to the behavior of the clients as the FL training progresses. As a result, tier-2 clients can move to tier-3 and vice-versa.



\subsection{Gathering Behavioral Data}
\label{sec:behavedata}
Our client selection strategy (\S\ref{sec:ClientSelection}) depends on the data collected from the clients' behavior in previous training rounds. Towards this, for each client we collect three attributes, i.e., \textit{training time}, \textit{missed rounds}, and \textit{cooldown}. \textit{Training time} is the time taken by the client to complete local model training. \textit{Missed rounds} is a list that contains the round numbers of the rounds missed by a client. We use this to calculate a client's penalty as described in \S\ref{sec:ClientSelection}. \textit{Cooldown} represents the number of rounds a client has to stay in the last tier and cannot participate in clustering (\S\ref{sec:tiers}). We evaluate the cooldown period from the client’s last missed round using Equation~\ref{eq: cooldown}. For instance, if a client missed round $2$, the cooldown is set to $1$. Moreover, if the same client missed round $4$, the cooldown is multiplied by two. As a result, the clients with \textit{cooldown} greater than zero are characterized as \textit{stragglers}. Towards this, using \textit{cooldown} can reduce the impact of temporarily slow or unavailable clients by lowering their priority for a certain number of rounds (\S\ref{sec:tiers}, \S\ref{sec:ClientSelection}).

\begin{footnotesize}
\begin{equation}
    cooldown = \left\{
     \begin{array}{@{}l@{\thinspace}l}
      0  &: \text{if the client completed training in time}\\
      1 &: \text{if cooldown = zero }\\
      cooldown \times 2 &: \text{otherwise}\\
     \end{array}
  \right.  
  \label{eq: cooldown}
\end{equation}
\end{footnotesize}


To gather and update the different client attributes, we modify the \emph{FedLess} controller (\S\ref{sec:sysdesign}) and FL client routines as shown in Algorithm~\ref{alg:client-side}. In each FL training round, the controller runs the \texttt{Train\_Global\_Model} routine, while the clients run the \texttt{Client\_U\-pdate} routine to locally train the model. \textit{nClientsPerRound} represents the maximum number of clients that must be selected in every round and \textit{maxRounds} represents the maximum number of allowed training rounds. 

Initially, the controller selects a subset of clients, invokes them, and then waits until they finish or a timeout occurs (Lines 3-4). Following this, we iterate over each successful client response and reset the \textit{cooldown} variable (Lines 5-8). Since the controller doesn't know if the client was slow or crashed, it assumes that the remaining invoked clients failed to finish. Subsequently, we update their \textit{missed rounds} and \textit{cooldown} attributes (Lines 9-12). At the client-side, we first load its behavioral history from previous rounds (Line 17). Following this, we measure the time for the client to load the global model, its local dataset, and train the model with its local data (Lines 18-21). Following this, each client sends its local model updates to the database (Line 22) and updates its training time for the current round (Line 23). Furthermore, slower clients that finished a round later can correct information about their missed rounds. As described before, the controller considers clients that did not finish the round in time as crashed. Therefore, distinguishing between crashed and slow clients is done on the client side. This is done by deleting the current round from their missed rounds list (Lines 24-26). Finally, the client updates its information in the database (Line 27).


% With FedLess~\cite{fedless}, each client stores its data in a corresponding storage bucket.

% In our strategy, we utilize clustering 

% Our strategy separates 

% Our selection scheme considers separating reliable clients that do not miss their training
% round from stragglers.

% owards this, for each client we collectg

% The client selection scheme relies on data collected on clients' behavior in previous rounds. Our selection scheme considers separating reliable clients that do not miss their training round from stragglers. Furthermore, we use clustering to partition the reliable clients into subsets with similar behavior. This means clients with similar performance are called in the same round to decrease waiting time at the controller and increase the system's efficiency. That said, we divide clients into three tiers. The first tier is for clients which never participated in a training round. We use this tier to make sure that each client has a chance to participate at least once to collect data about their behavior. The second tier includes reliable clients which participated in training at least once before. 
% The clustering is limited to the second-tier clients. Clustering these clients aims to group clients who behave similarly to improve system efficiency and reduce round time. We explain the details of clustering the second-tier clients in the next section. The last tier contains inconsistent clients which miss one or more successive rounds. The last-tier clients are not permitted to participate in the clustering. Clients are chosen from the last tier only if all clients from the first two tiers have been chosen and the required number of participants is not met.


%  The selection strategy relies on the following attributes to use in the clustering:
% \begin{itemize}
%     \item \emph{training time}: time taken by the client to finish training.
%     \item \emph{missed rounds}: a list that contains the round number of all missed rounds. In the next section, we discuss the usage of missed rounds to evaluate the client's penalty.
% \end{itemize}

% Moreover, each client has a \emph{cooldown} variable, which represents the number of rounds a client has to stay in the last tier. We evaluate the cooldown period from the client's last missed round. For instance, if client A missed round 2, the cooldown is set to 1. In this case, client A must stay in the last tier for one more round (round 3) before returning to the second tier in round 4. If client A missed round 4 (assuming client A is selected), the cooldown is multiplied by two. Consequently, client A has to stay in the last tier for two rounds. Equation \ref{eq: cooldown} shows how the cooldown variable is updated. Using this variable prevents wasting time and resources on calling clients which fail repeatedly. It can also reduce the impact of temporarily slow or unavailable clients by lowering their priority for a certain number of rounds.



% \begin{adjustbox}{width=8cm,center}
% \begin{equation}
%     cooldown = \left\{
%      \begin{array}{@{}l@{\thinspace}l}
%       0  &: \text{if the client completed training in time}\\
%       1 &: \text{if cooldown = zero }\\
%       cooldown \times 2 &: \text{otherwise}\\
%      \end{array}
%   \right.  
%   \label{eq: cooldown}
% \end{equation}
% \end{adjustbox}




% Algorithm~\ref{alg:client-side} shows the steps taken by the \acrshort{fedless} controller and client function to update the clients' attributes and how we distinguish between crashed and slow clients. \acrshort{fedless} controller runs the $Train\_Global\_Model$ function to train the global model for a single round. \acrshort{fedless} Clients run $Train$ function to train their local model. We define $n\_r$ as the number of clients that must be selected every round and $maxRounds$ as the maximum number of training rounds allowed. 

% At the \acrshort{fedless} controller, we select a subset of the clients and wait until they finish, or a timeout occurs (lines 2-3). We explain the details of the $Select\_Clients$ function in the next section. Then we iterate over each successful response for which we reset the cooldown variable (lines 5-8). Because \acrshort{fedless} controller does not know if a client is slow or ultimately crashed, it assumes that the remainder of the invoked clients failed to finish. Accordingly, we update their attributes in which the current round is recorded in the missed rounds list (line 10), and the cooldown is updated according to Equation \ref{eq: cooldown} (line 11-15).

% The $Client\_Update$ function shows the training flow at the client-side. We start by loading the client's behavioral history in the previous rounds (line 22). Afterward, we start to record the start time before loading the model and dataset (lines 23-25). Next, the client function trains the model on the local data (line 26). We record the training time at the end of training (line 27). The local model updates are sent to the parameter server (line 28). Clients are then required to update their training time for the current round (line 29). Furthermore, slower clients have a chance to correct information about their missed rounds if they finish the round later. As previously stated, the controller considers clients that did not finish the round in time as crashed. Therefore, distinguishing between slow clients and crashes is done on the client-side. We do that by allowing clients to correct assumptions made by the controller and erase the current round from their missed rounds list (lines 30-32).



% As per our three-tier division, we can define clients in order of their tier:
% \begin{enumerate}
%     \item \emph{rookies} (first-tier): which were not called before and yet to participate in training.
%     \item \emph{participants} (second-tier): which are allowed to participate in the clustering.
%     \item \emph{stragglers} (third-tier): which missed one or more successive rounds ($cooldown \ge 0$).
% \end{enumerate}

% We ensure that all clients have an opportunity to participate at least once at the start of the training by giving \textit{Rookies} the highest priority in our selection scheme. This method also allows us to collect behavioral data on all participants, which can be used for clustering in subsequent rounds. As the training progresses, the number of rookies decreases until it reaches zero, when all clients have been invoked before. \textit{participants} represents the clients ready to participate in the training round. During training, reliable clients are labeled as participants and are clustered based on their previous behavior. \textit{Stragglers} have the least priority.


% \subsection{Clustering-based Client Selection}
% \subsection{Selecting clients with clustering}

\begin{footnotesize}
\begin{equation}
  totalEma = trainingEma + missedRoundEma \times maxTrainingTime
 \label{eq:total-ema}
\end{equation}
\end{footnotesize}

\input{alg/client_selection}

\subsection{Selecting Clients}
\label{sec:ClientSelection}

% \todomc{Make algo more clearer}
Algorithm~\ref{alg:client-selection} describes our strategy for client selection in a particular FL training round. Our strategy promotes fair selection for reliable clients while involving stragglers less in the training process. Initially, we characterize the clients as \textit{rookies}, \textit{participants}, or \textit{stragglers} (\S\ref{sec:tiers}) based on their previous behaviour (Line 2). First, we randomly select the required number of clients in a round from the pool of \textit{rookie} clients. If the number of available \textit{rookie} clients is greater than the number of required clients, the algorithm terminates (Line 3-5). If not, we calculate the number of clients required from the \textit{participants} and the \textit{stragglers} (Lines 6-7). Note that, clients from \textit{stragglers} are only selected if the number of clients selected from the first and second tiers is not sufficient. Following this, we randomly sample the required number of straggler clients from the \textit{stragglers} (Line 8).
% explain the algorithm in action

% \todomohamed{add a line here about why we always select rookies first}
The reason for prioritizing rookies first is to guarantee that every client gets a chance to contribute to the global model. Moreover, it provides data on clients' behavior which is used to cluster clients in future rounds. Note that the number of rookies decreases as the training progress, until it reaches zero. In this case, the algorithm fully relies on the dynamic clustering of tier two clients.


% \begin{footnotesize}
% \begin{equation}
%   totalEma = sum\left(trainingEma, missedRoundEma*maxTrainingTime\right)
% \label{eq:total-ema}
% \end{equation}
% \end{footnotesize}

For the clients that will participate in clustering, we calculate two features. First, \textit{trainingEma} which represents an exponential moving average (EMA)~\cite{ema} on the previously recorded training times (Line 11). We use EMA since a weighted average better represents the current behavior of the client by giving higher weight to the recently recorded times. Second, \textit{missedRoundEma} which is a penalty factor based on the previous rounds missed by the client ~(\S\ref{sec:behavedata}). This satisfies two objectives. First, recent failures should have higher penalties. Second, the penalty should decrease as the training progresses if the client becomes more reliable. To compute \textit{missedRoundEma}, we divide the round numbers in the \textit{missed rounds} list by the current round number to get a list of ratios. Following this, we take an EMA on the computed ratios (Line 12). As the training progresses, the effect of a specific missed round decreases because the current round number increases. The computed features are added to the data required for clustering (Line 13). Following this, we use the collected data as input to the  \texttt{DBSCAN}~\cite{dbscan} algorithm for partitioning it into separate clusters, each with a specific label (Line 15). For generating clusters, \texttt{DBSCAN} relies on an $\epsilon$ parameter that represents the maximum distance between two samples to be considered in the neighborhood of each other. For simplicity, we treat outliers as a single cluster. To find a value for $\epsilon$, we do a grid search and select the parameter value that yields the highest \textit{Calinski-Harabasz index}~\cite{ch-index}. This score measures the ratio between intra-cluster and inter-cluster dispersion to evaluate the quality of the clusters. We chose this index because it is fast to compute and will not impact our running time. Moreover, due to the low time complexity of \texttt{DBSCAN}, i.e., \texttt{O(Nlog(N))} the time for computing clusters multiple times is insignificant compared to the overall round time. Following this, we sort the clusters according to the increasing order of the average \textit{totalEMA} of their members (Line 16). We calculate the \textit{totalEMA} using Equation~\ref{eq:total-ema}. For sampling clients from the sorted clusters, we start by first choosing the clients belonging to the faster clusters and gradually move to the slower clusters in the sorted list. Moreover, to provide maximum information to the global model and avoid sampling from the same cluster in every training round, we start choosing from the cluster corresponding to our current
training progress. This is determined by using the ratio between the
current round and the maximum number of rounds. We continue sampling from the clusters until we reach the required number of clients or there are no more clients to choose from. Finally, our algorithm returns a list of clients selected from \textit{rookies}, clusters, and \textit{stragglers}. 

% \todomc{Explain sampling clients from clusters}





% Algorithm~\ref{alg:client-selection} shows the pseudo-code for our selection scheme. The algorithm promotes fair selection for reliable clients while involving stragglers less in the training process. We start by selecting from the pool of rookie clients. The selection is made randomly if the pool is large enough until the remaining rookies are less than the required number of clients per round $(n\_r)$ (lines 6-8). We determine the number of clients selected from the second tier ($n\_c$) by subtracting the number of remaining rookies from $(n\_r)$ (line 9). Furthermore, we record the round $(s\_c\_r)$ in which we begin sampling tier 2 clients to use it later to choose which cluster to train (lines 10-12). If the clients selected from the first and second tiers are not enough, we randomly select the remaining clients $(s\_clients)$ from the third tier (lines 13-14).
 
%  For clients which will participate in clustering, we obtain two attributes. First, \textit{trainingEma} which represents an \acrfull{ema} on the previously recorded training time (line 17). Using a weighted average better represents the current client behavior by giving higher weight to the recent recorded times. Second, $(m\_r\_ema)$ which is a penalty factor based on previous missed rounds. This factor should satisfy two objectives. First, recent failures should have higher penalties. For instance, A client which failed in the second round would have a higher penalty than a client which failed in the first round. Second, the penalty should fade as we progress in training if the client becomes more reliable. In other words, if a client only missed the first round, the calculated client's penalty in round five must be less than its penalty in round two. To achieve this, we divide the numbers in the missed rounds list by the current round number to get a list of ratios (line 18). As the training progresses, the effect of a specific missed round decreases because the current round number increases. We then compute the missedRoundEma as an \acrshort{ema} on the computed list of the missed rounds (line 19).
 
% %% db_cluster explained
% After collecting the data for the participating clients, we use it to cluster the clients. The $DBScanClustering$ function partitions the clients' data into separate clusters, each with a specific label (line 22). \acrshort{dbscan} requires $\epsilon$ parameter to be set. For simplicity, we treat outliers as a single cluster. Although developers can tune the clustering parameters manually, we provide a simple method to pick the best-performing parameters. $DBScanClustering$ perform a grid search for the best parameter values that yield the highest \textit{Calinski-Harabasz index}~\cite{ch-index}. This score measures the ratio between intra-cluster and inter-cluster dispersion to evaluate the quality of the clusters. We chose this index because it is fast to compute; therefore, it will not affect our running time. Moreover, the low time complexity of \acrshort{dbscan} means that the time needed to run the clustering multiple times takes a few seconds, which is insignificant compared to the overall round time. Instead of developing the clustering algorithm from scratch, we rely on the \acrshort{dbscan} implementation provided by \textit{scikit- learn} library~\cite{dbscan-sklearn}.

%  The next step involves sorting the clusters according to the average total time of their members, where the total time of a client is the sum of its training time and its penalty time, as shown in Equation \ref{eq: total-ema} (line 23).
 
%  \begin{equation}
%   totalEma = time\_ema + (m\_r\_ema) \times maxTrainingTime
%   \label{eq: total-ema}
% \end{equation}

%  We then select clients according to the \textit{Sample} function(line 24). 


 
%  The \textit{Sample} function exists to select clients from the list of sorted clusters. Instead of randomly selecting clusters to run, we start by running the fastest clusters earlier in the training process. Then, we gradually move to slower clusters further in the sorted list. That way, faster clients serve as a hot start for the slower clients. As shown in Equation~\ref{eq: cluster-dx}, we choose the cluster corresponding to our current training progress. The current progress is determined using the ratio between the current round and the maximum number of rounds.
%   If the selected cluster size is more than the number of clients required, we sample clients from the selected cluster prioritizing the ones involved less in training; otherwise, we select the whole cluster. We update the required number of clients in both cases by subtracting the number of selected clients. As long as we do not reach the required number of clients, we move to the next cluster and repeat the same process. If we reach the end of the final cluster, we return to the first cluster in the list.
%   \begin{equation}
%   cluster\_idx = percentile((round - s\_c\_r)/ max(maxRounds - s\_c\_r, 1), sortedClusters)
%   \label{eq: cluster-dx}
% \end{equation}
 
%  The returned list of clients contains rookie clients, if any, appended to the selected clients from clustering and the list of stragglers that are selected to complete the required number of clients (line 25).

% \todonils{How our strategy is tailored for FaaS enviornments? 2-3 sentences}
\texttt{FedlesScan} accounts for offline clients and cold starts by not only relying on training time in the selection, but also by utilizing a dynamic penalty factor that accounts for delays and cold starts if they cause clients to miss their rounds. Furthermore, our strategy does not need any further computation on the client side, requiring clients to only be active during training making it suitable for serverless environments~(\S\ref{sec:stragglersfl}). 
% \todonils{accounting for cold starts behavior}
% \todoany{Elaborate on the explanation in the last paragraph}

\begin{footnotesize}
\begin{equation}
 w_{t+1} \longleftarrow \sum_{k=1}^{K} \frac{t_k}{t} \times \frac{n_{k}}{n} w^k_{t_k} 
 \label{eq:fedless-aggr}
\end{equation}
\end{footnotesize}

\subsection{Staleness-aware Aggregation}
\label{sec:stalelessaware}
Although our intelligent client selection strategy (\S\ref{sec:ClientSelection}) improves the efficiency of the system, stragglers are not completely eliminated. Stragglers might push their local model updates to the parameter server after the completion of an FL training round. Moreover, these updates might contain valuable information that can improve the performance of the global model. Towards this, we aggregate the delayed updates of the clients with a dampening effect asynchronously, i.e., delayed updates are considered the next time the aggregation function is called. 
Equation~\ref{eq:fedless-aggr} shows our updated aggregation function used to include stale updates. $w^k_{t_k}$ is the local model of client \textit{k} at round $t_k$ and $w_{t+1}$ is the global model after aggregation at round $t$. Furthermore, $n_k$ represents the cardinality of the dataset at client $k$ while $n$ is the total cardinality of the aggregated clients.  If the updates arrive at the same round ($t_k = t$), the equation becomes similar to \texttt{FedAvg}~\cite{mcmahan2017communication}. On the other hand, older updates ($t_k < t$), are dampened by $\frac{t_k}{t}$. To avoid obsolete updates from affecting the training, the aggregator uses a parameter $\tau$ to dictate the maximum age of updates included in the aggregation. Updates with $t - t_k \ge \tau$ are discarded by the aggregator. In our experiments, we use a value of two for $\tau$.
% To this end, we use a staleness-aware aggregation scheme to transform \texttt{FedLessScan} to a semi-asynchronous strategy.


% In the previous section, we discussed our intelligent selection strategy. Although an informed selection mechanism should improve the system's efficiency, slow clients will still be in the system. Therefore, we use a staleness-aware aggregation scheme to convert \acrshort{fedlesscan} to a semi-synchronous strategy. In \acrshort{fedless}, slow clients might push their updates after the round ends. Usually, these updates are considered wasted contributions. Furthermore, client updates might still hold valuable information to improve the model's performance. Our approach to tackling this problem enables the aggregator to include stall updates with a dampening effect. Equation~\ref{eq:fedless-aggr} shows the updated aggregation function used to include stale updates. Notice that $w^k_{t_k}$ is the local model of client \textit{k} at round $t_k$ and $w_{t+1}$ is the global model after aggregation at round $t$. Furthermore, $n_k$ represents the cardinality of the dataset at client $k$ while $n$ is the total cardinality of the aggregated clients. If the updates arrive at the same round ($t_k = t$), the equation becomes the same as Equation~\ref{eq:fedavg-client}. On the other hand, older updates ($t_k < t$), are dampened by $\frac{t_k}{t}$. To avoid obsolete updates from affecting the training, the aggregator uses a parameter $\tau$ to dictate the maximum age of updates included in the aggregation. Updates with $t - t_k \ge \tau$ are discarded by the aggregator.





==> sections/06_evaluation.tex <==
\subsection{Experiment Setup}


\subsubsection{Datasets}
\label{sec:datasets}
For our experiments, we use four datasets from different domains. These include image classification, i.e., (\textit{MNIST}~\cite{lecun-mnist}, \textit{FEMNIST}~\cite{cohen2017emnist}), language modeling, i.e., (\textit{Shakespeare}~\cite{shakespeare-gutenberg}), and speech recognition, i.e.,  (\textit{Google Speech}~\cite{speech}).


The MNIST handwritten Image Database consists of 60,000 images for training and 10,000 images for central evaluation. Similar to~\cite{fedless,mcmahan2017communication}, for simulating a non-IID setting, we sort the images by label, split them into 300 shards of 200 images each, and distribute the shards to the clients. We choose the FEMNIST and the Shakespeare datasets from a benchmarking framework for FL called \texttt{LEAF}~\cite{caldas2018leaf}. The FEMNIST dataset contains more than eight hundred thousand images, with an average of 226 images per client partition. The Shakespeare dataset contains sentences from \textit{The Complete Works of William Shakespeare}~\cite{shakespeare-gutenberg}. It is divided such that each role in each play is mapped to a specific partition. With more than four million samples, each of length 80 characters, a client is responsible for an average of 3743 samples. For this dataset, the task is to predict the next character in a sentence given the previous 80. We chose the real-world Google Speech dataset from the \texttt{FedScale}~\cite{fedscale} benchmark suite. This dataset was designed to build basic and helpful voice interfaces for applications with common words such as "Yes", "No," and directions. The primary goal of the speech recognition task is to train and evaluate keyword spotting systems to detect when a specific keyword is spoken~\cite{speech}. The dataset contains 105,000 samples of 1-second audio files distributed across 2618 clients. Out of the 2618 clients, $2168$ clients are for training, while the rest are for validation and testing. However, in our experiments we scale down the number of clients by four by using a custom mapping algorithm. As a result, we used 542 clients for the Google Speech dataset with each client containing training data of four corresponding clients from \texttt{FedScale}. 

% Note that, datasets from \texttt{LEAF} and \texttt{FedScale} are by default non-IID.



% to scale down the number of clients in our experiments, we implemented 

% The MNIST Handwritten Image Database~\cite{lecun-mnist} comprises 70,000 images of handwritten digits with ten classes corresponding to the respective digits. We use all 10,000 test images of the dataset to evaluate the global model after each training round centrally. To simulate a non-IID setting as in \cite{Chadha2020,mcmahan2017communication},
% we sort the 60,000 images in the training set by label, split them into 200 shards of 300 images each, and distribute the shards to the clients. This dataset represents an image classification task. 

% For our experiments, we rely on four datasets from 4 different benchmarks. We pick different domains to make the evaluation conclusive to test the new strategy. These domains include image classification (MNIST, FEMNIST), speech recognition (Google Speech), and language modeling (Shakespeare). 

% The first dataset is MNIST Handwritten Image Database. It contains 60000 images available for training and 10000 for central evaluation. The images are sorted and randomly distributed to 300 clients.

% We chose two datasets from \textit{LEAF}~\cite{leaf} which is a benchmarking framework for \acrshort{fl}. It contains a variety of datasets that cover different domains. 
% As per the original setup covered in~\cite{fedless}, we use both the FEMNIST dataset for image classification and the Shakespeare dataset for character prediction. FEMNIST is short for Federated Extended MNIST, which is based on splitting the Extended MNIST dataset~\cite{emnist}. The dataset contains more than eight hundred thousand images, with an average of 226 images per partition. Shakespeare dataset contains sentences from \textit{The Complete Works of William Shakespeare}~\cite{complete-work-sh}. The dataset is partitioned such that each role in each play is mapped to a specific partition. With more than four million samples, each of length 80 characters, a device is responsible for an average of 3743 samples.


% The last benchmark is \textit{FedScale}~\cite{fedscale}, which contains a group of large-scale realistic benchmark datasets for tasks such as object detection, word prediction, and speech recognition. From FedScale, we choose real-world speech recognition represented by the Google Google Speech dataset~\cite{speech}. The dataset was designed to build basic and helpful voice interfaces for applications with common words such as "Yes", "No," and directions~\cite{speech}. The dataset contains \num[group-separator={,}]{105000} samples of 1-second audio files distributed across 2618 clients. One of the challenges we faced with the Fedscale benchmark is that their implementation uses Pytorch~\cite{pytorch} while \acrshort{fedless} is based on Tensorflow~\cite{tensorflow}. Furthermore, the dataset is split using client-data mapping, which maps file ids to a particular client. The dataset was designed to be split into 2618 clients, 2168 of which are for training and the rest for validation and testing. Accordingly, we reimplemented the preprocessing scripts for the Google Speech dataset. Moreover, we implemented a custom mapping algorithm to scale the number of clients down according to a specific ratio. For example, a ratio of 4 means that one \acrshort{fedless} client is responsible for the training data of 4 FedScale clients. In our experiments, we used a ratio of 4 to map 542 \acrshort{fedless} clients to 2168 Fedscale clients.

%discuss the process if necessary.


\subsubsection{Model Architectures and Parameters}
\label{sec:models}
For each dataset, we use a DNN model architecture suited for the particular task. For the MNIST, FEMNIST, and the Shakespeare datasets, we use the same model architecture used in ~\texttt{LEAF}~\cite{caldas2018leaf}. On the other hand, for the Google Speech dataset we use a relatively simpler model as compared to the one described in \texttt{FedScale}~\cite{fedscale}. However, with our model we achieve similar results for accuracy as compared to~\cite{fedscale}. 


% \begin{table}[t]
% \centering
% \begin{tabular}{|c|cccc|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c|}{\textbf{Hyper Parameters}}                                                                                                     \\ \cline{2-5} 
%                                   & \multicolumn{1}{c|}{\textbf{Epochs}} & \multicolumn{1}{c|}{\textbf{Batch Size}} & \multicolumn{1}{c|}{\textbf{Optimizer}} & \textbf{Learning Rate} \\ \hline
% MNIST                             & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{10}                  & \multicolumn{1}{c|}{Adam~\cite{adam}}               & 0.001                  \\ \hline
% FEMNIST                           & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{10}                  & \multicolumn{1}{c|}{Adam}               & 0.001                  \\ \hline
% Shakespeare                       & \multicolumn{1}{c|}{1}               & \multicolumn{1}{c|}{32}                  & \multicolumn{1}{c|}{SGD~\cite{sgd}}                & 0.8                    \\ \hline
% Speech Command                    & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{5}                   & \multicolumn{1}{c|}{Adam}               & 0.001                  \\ \hline
% \end{tabular}
% \caption{Model hyperparameters used for each dataset.}
% \label{tab:hyperparams}
% \end{table}


% \begin{table}[t]
% \caption{Model hyperparameters used for each dataset.}
% \centering
% % \begin{adjustbox}{width=5.5cm,center}
%       \begin{tabular}{|>{\centering\arraybackslash}m{0.5cm}|>{\centering\arraybackslash}m{1.5cm}| >{\centering\arraybackslash}m{0.65cm}|>{\centering\arraybackslash}m{1.25cm}|>{\centering\arraybackslash}m{1.25cm}|}
%       \hline
%         \textbf{Dataset} & \textbf{Epochs} & \textbf{Batch Size} & \textbf{Optimizer} & \textbf{Learning Rate} \\ \hline 
%         MNIST & $5$ & $10$ & Adam~\cite{adam} & $1e-3$ \\ \hline
%         FEMNIST & $5$ & $10$ & Adam~\cite{adam} & $1e-3$ \\ \hline
%   \end{tabular}
    
% %  \end{adjustbox}
%  \label{tab:esp_benchmark}
% \end{table}


% For MNIST, we use a 2-layer Convolutional Neural Network (CNN) with a 5x5 kernel. Each convolutional layer is followed by a 2x2 max-pooling layer.  The model ends with a fully-connected layer with 512 neurons and a ten-neuron output layer. The model
% consists of 582,026 trainable parameters. Similarly, for FEMNIST we use a 2-layer CNN with a 5x5 kernel in which each convolutional layer is followed by a 2x2 max-pooling layer. The CNN layers are followed by a fully-connected layer with 2048 neurons, which is followed by an output layer with 62 neurons. Our model for FEMNIST contains a total of 6,603,710 trainable parameters. For the Shakespeare dataset, we use a Long Short Term Memory (LSTM) recurrent neural network~\cite{hochreiter1997long}. The model consists of an embedding layer of size eight followed by two LSTM layers with 256 units and an output layer of size 82. The final model contains 818,402 total trainable parameters. Our model architecture for Google Speech consists of two identical blocks followed by an average pooling layer and an output layer with 35 neurons. A block contains two convolutional layers with a 3x3 kernel followed by a max-pooling layer. A dropout layer follows the max-pooling layer with a rate of \texttt{0.25} to avoid overfitting. This results in 67,267 total trainable parameters for the model. 

For MNIST, we use a 2-layer Convolutional Neural Network (CNN) with a 5x5 kernel. Each convolutional layer is followed by a 2x2 max-pooling layer.  The model ends with a fully-connected layer with 512 neurons and a ten-neuron output layer. Similarly, for FEMNIST we use a 2-layer CNN with a 5x5 kernel in which each convolutional layer is followed by a 2x2 max-pooling layer. The CNN layers are followed by a fully-connected layer with 2048 neurons, which is followed by an output layer with 62 neurons. For the Shakespeare dataset, we use a Long Short Term Memory (LSTM) recurrent neural network~\cite{hochreiter1997long}. The model consists of an embedding layer of size eight followed by two LSTM layers with 256 units and an output layer of size 82. Our model architecture for Google Speech consists of two identical blocks followed by an average pooling layer and an output layer with 35 neurons. A block contains two convolutional layers with a 3x3 kernel followed by a max-pooling layer. A dropout layer follows the max-pooling layer with a rate of \texttt{0.25} to avoid overfitting. For MNIST, FEMNIST, and Google Speech, we use Adam~\cite{adam} as the optimizer with a learning rate of $1e-3$. On the other hand, for Shakespeare, we use SGD~\cite{sgd} with a learning rate of $0.8$. The clients for the MNIST, FEMNIST, and Speech datasets train for five local epochs with a batch size of $10$, $10$, and five respectively. Due to the limitations of the current commercial FaaS platforms (\S\ref{sec:faas}), the clients for Shakespeare train for one local epoch with a batch size of $32$. The hyperparameters for the different datasets are shown in Table~\ref{tab:experiment-params}.

% For all models, the output layer uses the softmax activation function, while all other layers use ReLU~\cite{agarap2018deep}. For the MNIST, FEMNIST, and Shakespeare models, we use \texttt{sparse\_categorical\_cr\-ossentropy} as the loss function, while for the Google Speech model we use \texttt{categorical\_crossentropy}. 




% The output layer uses softmax as the activation function while all other layers use ReLU~\cite{agarap2018deep}. 


% layer with softmax as the activation function.

% Each experiment trains a different model suited for the task. For MNIST, FEMNIST, and Shakespeare, we use the same model architecture mentioned by~\cite{fedless} and used in the original LEAF benchmark paper~\cite{leaf}. For MNIST, we use a 2-layer CNN with a 5x5 kernel. A 2x2 max-pooling layer follows each Convolutional layer. The model ends with a fully-connected layer with 512 neurons and a ten-neuron output layer with softmax activation. The model had a total of \num[group-separator={,}]{582026} trainable parameters.

% We picked two datasets from the LEAF benchmark. For FEMNIST, we use a 2-layer CNN with a 5x5 kernel. A 2x2 max-pooling layer follows each Convolutional layer. The model ends with a fully-connected layer with 2048 neurons followed by an output layer of 62 neurons with softmax activation. The final model contains \num[group-separator={,}]{6603710} trainable parameters.

% We use a Long Short Term Memory (LSTM) recurrent neural network~\cite{lstm} for the Shakespeare dataset. The model consists of an embedding layer of size eight followed by two LSTM layers with 256 units and an output layer of size 82 with softmax activation. The number of trainable parameters in the final model is \num[group-separator={,}]{818402}.

% For the FedScale benchmark, we opted for designing a simple CNN instead of replicating models from the FedScale benchmark itself. Since we are only interested in comparing different strategies, the designed model should show any differences if they exist. Nevertheless, the designed model was on-par with the results from the original FedScale paper~\cite{fedscale} in terms of accuracy. The model's architecture consists of two identical blocks followed by an average pooling layer and an output layer with 35 neurons, and a softmax activation. A block contains two convolutional layers with a 3x3 kernel followed by a max-pooling layer. A dropout layer follows the max-pooling layer with a rate of 0.25 to avoid overfitting. The number of trainable parameters in the model is \num[group-separator={,}]{67267}.

% To properly scale our experiments and eliminate database bottlenecks, we deployed the \acrshort{fedless} database on a single machine with 40vCPUs and 177GB of RAM. Furthermore, we use the same machine to run the \acrshort{fedless} controller. We deployed the aggregator function on a self-hosted single node OpenFaas cluster with 45GB of RAM and 10 vCPUs. The aggregation function had a memory limit of 7GB. Furthermore, we used a file server with 45GB of RAM, 10 vCPUs, and 200GB of storage to host the four datasets. 

% The client functions are deployed in the \textit{europe-west4} region due to the limited availability of $2^{nd}$ gen functions at the time of writing. Each client function had a memory limit of 2048MB and a maximum timeout of 540 sec. Table~\ref{tab:eval-clients} show the configuration we used for each dataset.  
% Because each dataset has a different number of clients, a single client runs on one function instance to ensure all clients can perform the training independently.

% \input{tab/dataset_client_config}

\input{tab/hyperparams}

\subsubsection{Experiment configuration}
\label{sec:expconfig}
To scale our experiments, we deployed \emph{FedLess} (\S\ref{sec:sysdesign}) on a VM hosted by the LRZ compute cloud~\cite{lrzcc}. The VM was configured with $40$ virtual CPUs (vCPUs) and $177$GB of RAM. For the aggregator function, we use a self-hosted OpenFaaS~\cite{openfaas} cluster deployed on a VM with 10vCPUs and 45GB of RAM. We limit the memory of the aggregation function to $7$GB. Furthermore, for hosting our datasets we use a nginx~\cite{nginx} store running on a VM with 10vCPUs and 45GB of RAM.

For all our experiments, we deployed the FaaS based FL clients on the 2$^{nd}$ generation GCFs~\cite{gcloud-functions-2} based on Knative~\cite{knative}. Each client function had a memory limit of 2048MB and a timeout of 540 sec. For the MNIST, FEMNIST, and Google Speech datasets, we use $200/300$, $175/300$, and $200/542$ concurrent clients per round respectively. On the other hand, for Shakespeare, we use $50/100$ clients per round.

\begin{figure*}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/eval/speech/wide/acc_speech.pdf}
\caption{Comparing Accuracy.}
\label{fig:acc-speech}
\end{subfigure}%
 \hfill

\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/eval/speech/wide/eur_speech.pdf}
\caption{Comparing \texttt{EUR}.}
\label{fig:eur-speech}
\end{subfigure}%
 \hfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/eval/speech/wide/var_speech.pdf}
% \caption{Distribution of client's invocation frequency on the Speech Commands dataset~\cite{speech}.}
\caption{Comparing the distribution of invocation frequency of clients.}
\label{fig:var-speech}
\end{subfigure}%
\caption{Comparing the different metrics for the different strategies on the Google Speech dataset~\cite{speech} with varying straggler ratios.}
\label{fig:metricsovertime}
\shrinkspace
\end{figure*}


\subsubsection{Experiment scenarios}
\label{sec:scenarios}
% To properly scale our experiments and eliminate database bottlenecks, we deployed the \acrshort{fedless} database on a single machine with 40vCPUs and 177GB of RAM. Furthermore, we use the same machine to run the \acrshort{fedless} controller. We deployed the aggregator function on a self-hosted single node OpenFaas cluster with 45GB of RAM and 10 vCPUs. The aggregation function had a memory limit of 7GB. Furthermore, we used a file server with 45GB of RAM, 10 vCPUs, and 200GB of storage to host the four datasets. 

% The client functions are deployed in the \textit{europe-west4} region due to the limited availability of $2^{nd}$ gen functions at the time of writing. Each client function had a memory limit of 2048MB and a maximum timeout of 540 sec. Table~\ref{tab:eval-clients} show the configuration we used for each dataset.  
% Because each dataset has a different number of clients, a single client runs on one function instance to ensure all clients can perform the training independently.
With our experiments, we aim to evaluate the performance of our strategy against delays and client function dropouts. Although the deployed functions will show delays, failures, and cold starts, it does not indicate how our strategy behaves in extreme situations, i.e., with a significantly high number of stragglers. Towards this, we consider two scenarios in our experiments.

\textbf{Standard Scenario}. In this, we perform the experiments on the deployed client functions without any modifications. Furthermore, we adjust the FL training round time to ensure that the clients can finish their training before the training round ends. This scenario demonstrates the performance in a more real-world situation when clients on commercial FaaS platforms are used for training.

% \textbf{Straggler (\%) Scenario}. In this, we simulate varying percentages of stragglers in the FL system.  Although there might be different reasons for FaaS client failures, such as memory limit, function timeout, or communication issues, these failures can only have one of two effects on the clients. Clients can either push their updates after the training round is finished (slow updates) or can completely crash (not push their updates). To simulate slow updates, we limit the training round time to only fit clients with no issues or delays. Meaning, that clients which experience cold starts, bandwidth limitations, or communication delays do not finish the round in time; therefore, pushing their updates later. On the other hand, to simulate failures, we randomly select a specific ratio of clients to fail their training at the beginning of each experiment. We perform four different experiments for each dataset with 10\%, 30\%, 50\%, and 70\% stragglers in the system. 


\textbf{Straggler (\%) Scenario}. In this, we simulate varying percentages of stragglers in the FL system.  Although there might be different reasons for FaaS client failures, such as memory limit, function timeout, or communication issues, these failures can only have one of two effects on the clients. Clients can either push their updates after the training round is finished (slow updates) or can completely crash (not push their updates). To simulate slow updates, we limit the training round time to only fit clients with no issues or delays. Meaning, that clients which experience cold starts, bandwidth limitations, or communication delays do not finish the round in time; therefore, pushing their updates later. On the other hand, to simulate failures, we randomly select a specific ratio of clients to fail their training at the beginning of each experiment. We perform four different experiments for each dataset with 10\%, 30\%, 50\%, and 70\% stragglers in the system. Note that, in all our experiments, stragglers are different from \textit{malicious clients} found in some FL settings~\cite{li2020learning, zhang2022fldetector}. While malicious clients can act as stragglers to deliberately slow training or hinder model performance, they can perform more powerful attacks such as data or model poisoning~\cite{fl_challenges,fl_data_poisoning} to skew the model's performance. In our work, we focus on the problem of stragglers and their behavior rather than the clients' intentions. The number of training rounds for the different datasets and experiment scenarios is shown in Table~\ref{tab:experiment-params}.

% Malicious clients are responsible for initiating attacks on the FL server leading to deterioration in the performance of the model or failure of model training. In contrast, all stragglers in our experiments are clients that have been authenticated and authorized by the \emph{FedLess} controller.

% \todoany{Write difference from malicious clients}

% \todonils{Add a line to make slow updates more clearer}
% We aim to evaluate the performance of \acrshort{fedlesscan} against delays and function dropouts. Although the deployed functions will show delays, failures, and cold starts, it does not indicate how our strategy behaves in extreme situations~\cite{fedless}. Therefore, we decided to test two separate scenarios. 

% In the standard scenario, we perform the experiments on the client function without any modifications. Furthermore, the round time is adjusted to ensure clients can finish their local training before the round ends. This scenario shows the performance in a more real-world situation when using \acrshort{faas} providers as an infrastructure base for the experiment. In subsequent sections, we refer to this experiment as the standard scenario.

% The second scenario includes synthesized experiments where we simulate multiple stragglers ratios in the system. Although there might be different reasons for client failure, such as memory limit, function timeout, or communication issues, simulating different failure types will significantly increase the experiment cost. These failures can only have one of two effects on the clients. Clients can completely crash (not push their updates) or push their updates after the training round is finished (slow updates).

% In order to simulate slow updates, we opted to strict the round time such that clients with cold starts will not finish before the end of the round. We considered simulating slow updates by introducing delays in the functions, but we found a significant increase in the experiment cost. To simulate failures, we randomly select a specific ratio of clients to fail their training at the beginning of each experiment. We perform four different experiments for each dataset with 10\%, 30\%, 50\%, and 70\% stragglers. We refer to the experiment by its stragglers' ratio in subsequent sections.

% With about 60 experiments, we analyze the results on each dataset separately and provide further insights on the behavior of \acrshort{fedlesscan} compared to \acrshort{fedavg} and \acrshort{fedprox}.

% \subsection{Accuracy and Client Utilization}

\input{tab/accuracy_analysis}






\subsubsection{Metrics}
\label{sec:metrics}
For comparing the different strategies, we use the standard metrics \textit{accuracy}, \textit{experiment duration}, and \textit{cost}. For calculating accuracy of the trained global model, we randomly choose a set of clients and evaluate it on their test datasets. Following this, we multiply the obtained accuracy for a particular client by the ratio of its test set cardinality to the total cardinality of the test dataset. The final accuracy value is obtained by averaging the obtained accuracy values. While accuracy describes model performance, it does not provide insights about the performance of the strategy and the contributions of the clients to the global model. Towards this, we also use the metrics \textit{Effective Update Ratio} (EUR)~\cite{safa} and \textit{Bias}~\cite{safa}. EUR is defined as the ratio between the successful clients and the subset of selected clients. It shows the effect of stragglers on round utilization. A higher value of EUR represents less wasted resources since clients requested to participate in a certain round end up contributing to the global model. Furthermore, to provide insights into the bias of the client selection schemes, we use variance plots. This is done by showing the frequency of selection for each client across the FL training process. Bias is defined as the difference between the frequency of the least called client and the most called client~\cite{safa}. For scenarios with low number of stragglers, we target low bias, while for scenarios with high number of stragglers the bias should be higher due to the prioritization of reliable clients in training. Experiment duration represents the total time required for training the model. For computing training costs, we use the cost computation model~\cite{gcf_cost} used by Google to estimate the cost for each client function based on the number of invocations, allocated memory, and execution duration.



% \todonils{Add a sentence why accuracy is not enough}
% Although accuracy describes the model performance, it does not reveal details about the strategy performance or the client contributions to the global model. 





\subsection{Comparing accuracy and round utilization}
\label{sec:accandutil}


% Table~\ref{tab:acc-all} provides a summary for both accuracy and \acrshort{eur} values across all our experiments. 
% In Standard scenarios, \acrshort{fedlesscan} showed better accuracy and round utilization. \acrshort{fedlesscan} outperformed both \acrshort{fedavg} and \acrshort{fedprox} on all datasets with the exception of Shakespeare dataset. Our analysis of the Shakespeare dataset shows that some of the clients might contribute to the model accuracy more than others, especially clients with longer training time. Moreover, the training session was slightly short, with only 25 rounds, due to budget constraints. We argue that in a more realistic scenario with more rounds, the difference in accuracy will decrease. 
 
The obtained accuracy and EUR values across all our experiments is summarized in Table~\ref{tab:acc-all}. For the \textit{standard scenarios} (\S\ref{sec:scenarios}), we obtained better accuracy and round utlization for our strategy as compared to \texttt{FedAvg} and \texttt{FedProx} across all datasets except Shakespeare. This is because with the Shakespeare dataset, some of the clients contribute to the model accuracy more than others, especially clients with longer training times. Moreover, due to budget constraints and significantly high training costs, we train for a slightly less number of rounds, i.e., 25 for Shakespeare. However, we argue that in a more realistic scenario with more number of rounds, the difference in accuracy will decrease. This is because our strategy utilizes clients more efficiently, i.e., higher EUR. As a result, with more rounds the number of invocations per client will increase and more clients will contribute to the global model, leading to a higher accuracy. Similarly, for the \textit{straggler (\%) scenarios}, we obtained better results for accuracy with our strategy as compared to the other two for the MNIST, FEMNIST, and the Google Speech datasets. On the Shakespeare dataset, our strategy outperformed \texttt{FedAvg} and \texttt{FedProx} in scenarios with 30\%, 50\%, and 70\% stragglers. In terms of EUR, our strategy constantly outperforms the other two strategies across all scenarios and datasets since they use random selection for selecting clients for an FL training round.

% For the \textit{straggler (\%) scenarios}, with our strate

% as the number of invocation per client will increase and given that we utilize clients more efficiently (higher EUR) more clients will contribute to the global model, enhancing accuracy at the end.
 
% In our simulated scenarios, \acrshort{fedlesscan} delivered better accuracy on MNIST, FEMNIST, and Google Speech datasets.
% On the Shakespeare dataset, \acrshort{fedlesscan} outperformed \acrshort{fedavg} and \acrshort{fedprox} in scenarios with 30\%, 50\%, and 70\% stragglers.
% From our results, we can define a proper usecase for \acrshort{fedlesscan}. Although \acrshort{fedlesscan} was designed as a straggler-resilient variation of \acrshort{fedavg} on serverless \acrshort{fl}, the strategy does not try and reduce or eliminate stragglers from the system. That said, \acrshort{fedlesscan} works best in long training sessions because there are more data collected about the clients' behavior that will help group clients better. In case of repeated failures, \acrshort{fedlesscan} should perform well due to its three-tier classification system. Furthermore, we notice that in the case of small-scale experiments with a small number of clients per round, strategies based on random client selection might perform better than \acrshort{fedlesscan}. We notice this effect in the Shakespeare experiment as the benefits of grouping clients with similar behavior appear in large-scale experiments.



% Furthermore, we observe that for small-scale experiments with a small number of clients per round, 

% The overall evaluation showed that \acrshort{fedlesscan} achieves an average of 2\% better accuracy in 8\% shorter round time and up to 20\% lower cost compared to \acrshort{fedavg} and \acrshort{fedprox}.


%%% show speech results


%%%%%% speech acc %%%%%%%%%%
% We further investigate the speech recognition task's performance of the Google Speech dataset from the FedScale benchmark. Figure~\ref{fig:acc-speech} depicts the accuracy over time comparison for the three strategies in both standard and synthesized scenarios. In the standard scenario, we ran the three strategies for 35 rounds. We see \acrshort{fedlesscan} outperform both \acrshort{fedavg} and \acrshort{fedprox} in terms of convergence rate and end accuracy. \acrshort{fedlesscan} reached an accuracy of 79.4\% compared to 76.6\% for \acrshort{fedavg} and 77.4\% for \acrshort{fedprox}.  Furthermore, \acrshort{fedlesscan} showed faster convergence by reaching an accuracy of 70\% in 19 rounds compared to 21 and 22 for \acrshort{fedprox} and \acrshort{fedavg} respectively. 



% \todomohamed{Explain why we obtain better accuracy than FedAvg and FedProx?.}

% \texttt{FedLesScan} obtained better accuracy in most \textit{standard scenarios} due to better distribution of client invocations by prioritizing clients with fewer contributions resulting in more balanced contributions among the participating clients. In \textit{straggler (\%) scenario}, we believe FedLesScan reached better accuracies by relying more on robust and reliable clients. Furthermore, the utilization of a staleness-aware aggregation scheme avoids wasting valuable contributions, which in turn boosts accuracy.

For most \textit{standard scenarios} (Table~\ref{tab:acc-all}), \texttt{FedLesScan} obtained better accuracy as compared to the other two strategies due to the better distribution of client invocations. This is because our strategy prioritizes clients with the least number of invocations in a selected client cluster (\S\ref{sec:ClientSelection}) leading to more balanced contributions among the participating clients. On the other hand, with \textit{straggler (\%) scenario}, our strategy reached better accuracies by relying more on robust and reliable clients. Furthermore, the utilization of a staleness-aware aggregation scheme (\S\ref{sec:stalelessaware}) avoids wasting valuable contributions, which in turn increases accuracy.

% MNIST: Acc increases with higher number of stragglers (FedAvg, FedLessScan)
% Shakespeare: Acc increases with higher number of stragglers  (FedAvg, FedLessScan),
% Google Speech: Acc increases with higher number of stragglers  (FedAvg, FedProx, FedLessScan).
% We need to come with a plausible explanation for this.}

% We noticed that the presence of stragglers affects the convergence speed such that the standard scenarios converge faster than \textit{straggler (\%) Scenarios}. Figure~\ref{fig:metricsovertime} depicts the difference in convergence rate between both scenarios by showing the accuracy over time for the google speech command dataset. Given the experiment hyper parameters in table~\ref{tab:experiment-params}, the \textit{standard scenario} reached a similar range of accuracy in 35 rounds compared to 60 rounds for the \textit{straggler (\%) scenarios}. The rest of the experiments on the remaining datasets show that the presence of stragglers affected the end accuracy, but not to the same extent as the google speech dataset. Moreover, in the \textit{straggler (\%) scenarios}, increasing the percentage of stragglers does not seem to cause a consistent decrease in accuracy, especially in straggler-heavy scenarios. This behavior is not exclusive to our experiments. Li et al.~\cite{fedprox} and Wu et al.~\cite{safa} documented similar behavior in their experiments. While they did not provide a clear explanation for this phenomenon, we argue that due to the non-IID nature of the data, clients do not contribute evenly to the test accuracy. In addition, it is easier to reach a consensus on a global model which represents a smaller number of clients; therefore, we can reach situations where a system with more stragglers reaches higher overall accuracy at the end.


% \todomohamed{rephrase last sentence}

\input{tab/time_analysis}

To offer detailed insights, we present results for the Google Speech dataset~\cite{speech} wrt the metrics accuracy and EUR, across the FL training session as shown in Figures \ref{fig:acc-speech} and \ref{fig:eur-speech} respectively. For the \textit{standard scenarios}, we ran the FL training session for $35$ rounds, while for the \textit{straggler (\%) scenarios}, we ran the experiments for $60$ rounds. For the standard scenario, our strategy reached an accuracy of 79.4\% as compared to 76.6\% and 77.4\% for \texttt{FedAvg} and \texttt{FedProx} respectively. Furthermore, our strategy showed faster convergence by reaching an accuracy of 70\% in 19 rounds as compared to 21 and 22 for \texttt{FedAvg} and \texttt{FedProx} respectively. With 10\% stragglers, our strategy and \texttt{FedAvg} had a similar convergence rate, while \texttt{FedProx} was slightly behind. Moreover, our strategy reached an end accuracy of 76\% which is a 6\% and 10\% increase over \texttt{FedAvg} and \texttt{FedProx} respectively. For an FL system with 30\% stragglers, our strategy consistently outperforms \texttt{FedAvg} by around 8\% towards the end of the training, while outperforming \texttt{FedProx} by a smaller margin of 1\%. We observe a similar trend for our experiments with 50\% and 70\% stragglers in the system, where our strategy outperforms the other two. From our experiments, we observe that the presence of stragglers affects the convergence speed of the DNN models in an FL training session. DNN models trained in \textit{standard scenarios} converge faster as compared to the models trained with \textit{straggler (\%) scenarios} as shown in Figure~\ref{fig:acc-speech} (Table~\ref{tab:experiment-params}). We observe a similar behaviour for the different datasets (\S\ref{sec:datasets}). Moreover, for the \textit{straggler (\%) scenarios}, increasing the percentage of stragglers in the system does not consistently decrease the accuracy of the trained DNN model as shown in Table~\ref{tab:acc-all}. This is especially true for experiments with a higher number of stragglers, i.e., $70\%$. This behavior is not exclusive to our experiments and was also reported by Li et al.~\cite{fedprox} and Wu et al.~\cite{safa}. While the authors do not provide a clear explanation for this behaviour, we argue that due to the non-IID nature of the data, clients do not contribute evenly to the test accuracy. In addition, having fewer number of reliable clients reduces the varying effect of local model updates and local model deviations from the global model, making it easier to reach a consensus on the global model. Therefore, we can reach situations where a system with more stragglers reaches higher overall accuracy at the end. 

% In addition, fewer number of reliable clients reduces local model deviations from the global model and the varying effect of local updates, making it easier to reach consensus on a global model. Therefore, we can reach situations where a system with more stragglers reaches higher overall accuracy at the end.


% To offer detailed insights, we present results for the Google Speech dataset~\cite{speech} wrt the metrics accuracy and EUR, across the FL training session as shown in Figures \ref{fig:acc-speech} and \ref{fig:eur-speech} respectively. For the \textit{standard scenarios}, we ran the FL training session for $35$ rounds, while for the \textit{straggler (\%) scenarios}, we ran the experiments for $60$ rounds. For the standard scenario, our strategy reached an accuracy of 79.4\% as compared to 76.6\% and 77.4\% for \texttt{FedAvg} and \texttt{FedProx} respectively. Furthermore, our strategy showed faster convergence by reaching an accuracy of 70\% in 19 rounds as compared to 21 and 22 for \texttt{FedAvg} and \texttt{FedProx} respectively. With 10\% stragglers, our strategy and \texttt{FedAvg} had a similar convergence rate, while \texttt{FedProx} was slightly behind. Moreover, our strategy reached an end accuracy of 76\% which is a 6\% and 10\% increase over \texttt{FedAvg} and \texttt{FedProx} respectively. For an FL system with 30\% stragglers, our strategy consistently outperforms \texttt{FedAvg} by around 8\% towards the end of the training, while outperforming \texttt{FedProx} by a smaller margin of 1\%. We observe a similar trend for our experiments with 50\% and 70\% stragglers in the system, where our strategy outperforms the other two.



% For the standard scenario, we observe that our strategy outperforms the other two strategies wrt convergence rate and end accuracy. 

% Our strategy reached an accuracy of 79.4\% as compared to 76.6\% and 77.4\% for \texttt{FedAvg} and \texttt{FedProx} respectively. Furthermore, our strategy showed faster convergence by reaching an accuracy of 70\% in 19 rounds as compared to 21 and 22 for \texttt{FedAvg} and \texttt{FedProx} respectively.

% For the straggler (\%) scenario, we ran the experiments for 60 rounds to see the long-term behavior of the three approaches on a real world-dataset. For the second plot with 10\% stragglers, \acrshort{fedlesscan} and \acrshort{fedavg} had a similar convergence rate while \acrshort{fedprox} was slightly behind. Furthermore, \acrshort{fedlesscan} reached an accuracy of 76\% which is a 6\% and 10\% increase over \acrshort{fedavg} and \acrshort{fedprox} respectively. 
% The third plot with the 30\% stragglers shows \acrshort{fedlesscan} consistently outperforming \acrshort{fedavg} by about 8\% towards the end of the training while outperforming \acrshort{fedprox} by a smaller margin of 1\%. Although \acrshort{fedprox} suffered a slight decline in accuracy towards the end of the training, it managed to outperform \acrshort{fedavg} at the end.
% The same trend continues for the rest of the synthesized experiments. In the 50\% stragglers scenario, \acrshort{fedlesscan} outperformed \acrshort{fedavg} and \acrshort{fedprox} by 7\% and 3\% respectively. In the last experiment with 70\% stragglers, \acrshort{fedavg} performed better compared to its previous results outperforming \acrshort{fedprox} by 1\%. Nevertheless, the end accuracy of \acrshort{fedlesscan} was higher than \acrshort{fedavg} by 3\%.
\input{tab/cost_analysis}

%%%%%%%%%%%%%%%%%%%%%% speech EUR
% \input{tab/cost_analysis}
 Figure~\ref{fig:eur-speech} shows the EUR comparison among the three strategies for the different scenarios. In the standard scenario, the three strategies performed similarly, achieving more than 99\% average EUR ratio during training. In the straggler (\%) scenarios, our strategy consistently achieves higher EUR as compared to the other strategies. Furthermore, as the number of stragglers in the system increases, the difference between the average EUR of our strategy as compared to the other two also increases. We observe occasional drops in EUR for our strategy with varying number of stragglers in the system. These drops demonstrate the effect of clustering of the clients. Distributing slow clients across the training rounds will affect the efficiency of more rounds. 
 
%  old 
%Our strategy, combines clients with similar behavior together, thereby decreasing the effect of stragglers on training the other clients. However, this leads to occasional drops in the EUR, while still maintaining a higher EUR value in the subsequent training rounds. 

% \todomohamed{Explain drops in EUR a bit better. Clarify that clustering happens in everyround right wrt the comments from Reviewer2}
Our strategy utilizes dynamic clusters to combine clients with similar behavior together. Recomputing the clusters each round based on clients'  recent behavior reduces the impact of stragglers on training the other clients. However, this leads to occasional drops in the EUR, which happens when an unreliable subset of clients is invoked. The subsequent rounds, involving the rest of the clients, maintain higher EUR values, thereby decreasing the total training time. 



%  Figure~\ref{fig:eur-speech} depicts the \acrshort{eur} comparison among the three strategies. In the standard scenario, the three strategies performed similarly, achieving more than 99\% average \acrshort{eur} ratio during training. In the straggler (\%) scenario, \acrshort{fedlesscan} consistently achieves higher \acrshort{eur} compared to the other strategies; we also see the gap increase as the ratio of stragglers increases. Furthermore, we notice occasional drops in \acrshort{eur} plots for \acrshort{fedlesscan}. These drops show the effect of clustering the clients. Distributing stragglers across the training rounds will affect the efficiency of more rounds. For instance, consider a system that contains ten stragglers. If the invocation of those ten stragglers is distributed among all rounds, there will be at least ten rounds affected by stragglers. These effects can lead to clients waiting for the straggler to finish, decreasing the system efficiency and increasing training duration. Alternatively, \acrshort{fedlesscan} combines stragglers with similar behavior together, decreasing their effect on training the other clients. This leads to occasional drops in the \acrshort{eur}, as seen in the plots, but it shows that the system can maintain a higher ratio in subsequent rounds.

%%%%%%%%%%%%% speech bias

% Although the \acrshort{eur} shows the efficiency of the system, it does not show the bias of the strategy. A system that utilizes a specific subset of clients and discards the rest of the clients will have high \acrshort{eur} but will underutilize the rest of the clients. The violin plots in Figure~\ref{fig:var-speech} provides us with further insights into the bias encountered by our strategy. The graph shows a distribution based on the number of invocations for each client (y-axis). We demonstrate bias by the difference between the highest and lowest point in the distribution. When the difference between the two points increases (the height increase), the algorithm is biased towards a specific subset of clients. On the contrary, when the height decreases, the difference between the most and least invoked clients is low. Furthermore, the width of the plot at a particular point X provides insights into the ratio of clients called X times. If the width at point X is larger than at an arbitrary point Y, then the number of clients called X times is more than the number called Y times. We rely on this explanation to understand the behavior of our strategy.
% \balance


Although EUR demonstrates the efficiency of the system, it does not show the bias of the strategy. A system that utilizes a specific subset of clients and discards the rest will have a higher EUR but will underutilize the rest of the clients. To this end, we use violin plots as shown in Figure~\ref{fig:var-speech} to provide insights into the bias encountered by our strategy (\S\ref{sec:metrics}). The graph shows a distribution based on the number of invocations for each client (y-axis). We demonstrate bias by the difference between the highest and lowest points in the distribution. A greater difference (height) represents that the algorithm is biased towards a specific subset of clients, while a smaller difference (height) represents that the difference between the most and least invoked clients is low. A bigger width indicates that certain clients were invoked more frequently. For the \textit{standard scenario}, we observe that \texttt{FedAvg} and \texttt{FedProx} show similar behaviour without distinguishing between stragglers and reliable clients. This is because they use random client selection. On the other hand, our strategy adapts to stragglers and promotes fair selection of clients. This is apparent since the distribution of our strategy is centered around similar values, i.e., most clients have the same number of invocations. Furthermore, we observe that with our strategy few clients have a low number of invocations. This is because clients that have repeatedly failed due to memory constraints are not used as often as the rest of the clients. For the \textit{straggler (\%) scenarios}, we observe that our strategy prioritizes reliable clients while relying on stragglers less during training. We see a distinction between the number of invocations of reliable clients and stragglers.

% As per the information discussed above, the graphs in Figure~\ref{fig:var-speech} show the bias encountered by our selection strategy. \acrshort{fedavg} and \acrshort{fedprox} use random client selection; therefore, they show similar behavior without distinguishing between stragglers and reliable clients. On the other hand, \acrshort{fedlesscan} dynamically adapts to stragglers. We see that the strategy promotes fair client selection in the standard scenario. We demonstrate this by comparing the height difference in each plot. We notice that the \acrshort{fedlesscan} plot is more concentrated in the middle, which means clients get an equal share of training. Furthermore, we observe that the \acrshort{fedlesscan} distribution shows few clients with a low number of invocations. This is because clients that have repeatedly failed due to memory constraints are not used as often as the rest of the clients

% In the synthesized scenarios, we see \acrshort{fedlesscan} prioritizing reliable clients while relying on stragglers less during training. We see a distinction between the number of invocations of reliable clients and stragglers.



%%%%%%%%%%%%%%%%%%


From our experiments, we observe that \texttt{FedLesScan} performs best in long FL training sessions due to the large amount of training data collected about the behaviour of the clients. The collected data leads to better groupings of the clients (\S\ref{sec:ClientSelection}). Moreover, in the case of repeated failures of clients, our strategy should perform well due to its three-tier classification system (\S\ref{sec:tiers}). 

% \todonils{This section needs to be reworked from the second paragraph, remove all references to plots of datasets, experiments we don't show. Start with explaining accuracy results of the Google Speech dataset, then EUR, then variance.}




\subsection{Comparing time and cost}
\label{sec:timecost}
Although model accuracy is an important metric, fast convergence wrt the number of training rounds does not provide a complete picture of the efficiency of the system. Towards this, in this section, we provide a collective analysis of all experiments wrt total duration and costs. To compute the total experiment duration, we aggregate the total round time during training. For all the three strategies, the round time is determined by the slowest invoked client. As a result, the round time depends on either the response of the slowest client or a predetermined timeout (\S\ref{sec:scenarios}). Furthermore, for \textit{straggler (\%) scenarios}, we simulate real-world behavior by assuming that the stragglers will not respond, thus forcing the controller (\S\ref{sec:sysdesign}) to wait until the round timeout. 

% For computing time, we use the maximum round timeout. 


% For all the three strategies, the round time is determined by the slowest invoked client. As a result, the round time is determined by either the response of the slowest client or a predetermined timeout (\S\ref{sec:scenarios}). Our calculations compute the total experiment time by aggregating the round time during training. Furthermore, for \textit{straggler (\%) scenarios}, we simulate real-world behavior by assuming that the stragglers will not respond, thus forcing the controller to wait until the round timeout. 

% Although accuracy is an essential factor, it does not inform us about the efficiency of the system or the strategy used. Furthermore, the accuracy results in the previous section were expressed in terms of the number of rounds. Fast convergence in terms of the number of rounds does not provide a complete picture of the system efficiency. This section provides a collective analysis of all experiments in terms of duration and cost.
% Time computation was done based on the maximum round timeout. In the three strategies, the round time is dictated by the slowest client invoked. Therefore, the round time is determined by either the response of the slowest client or a predetermined timeout. Our calculations compute the total experiment time by aggregating the round time during training. Furthermore, we simulate real-world behavior by assuming that stragglers in the synthesized scenarios do not respond, thus forcing the controller to wait until the round timeout. 


Table~\ref{tab:total-time} shows the total aggregated time per experiment. For the \textit{standard scenario}, training a model with our strategy is significantly faster as compared to \texttt{FedAvg} and \texttt{FedProx} across all datasets. For instance, for the MNIST dataset, our strategy takes 40\% less time as compared to the other strategies. For the \textit{straggler (\%) scenarios}, we see the effect of stragglers on experiment duration. In the scenarios with 10\% and 30\% stragglers, we observe that 
\texttt{FedLesScan} maintains a lower duration across all experiments. However, when the number of stragglers in the system is significantly higher, they must be invoked in almost all training rounds to meet the minimum number of clients required per round. We notice this behavior for our strategy with greater than 50\% stragglers in the system for the MNIST, FEMNIST, and the Shakespeare dataset. However, for the Google Speech dataset, our strategy still has an 18\% lower experiment duration as compared to the other two. This is because the total number of clients for the Google Speech dataset is 542 with 200 concurrent clients participating in a training round (\S\ref{sec:expconfig}). For the scenario with 70\% stragglers in the system, all approaches have similar experiment times across all datasets.
% Moreover, for the Google Speech dataset, our strategy


% Table~\ref{tab:total-time} shows the total aggregated time per experiment. In the standard scenario, the duration of the \acrshort{fedlesscan} is significantly shorter than \acrshort{fedavg} and \acrshort{fedprox} across all datasets. On the MNIST dataset, \acrshort{fedlesscan} had a 40\% lower duration than both strategies. On the FEMNIST dataset, our approach reached higher-end accuracy in 7\% less time compared to other approaches. On the Shakespeare dataset, \acrshort{fedavg} and \acrshort{fedprox} had 15\% longer duration than \acrshort{fedlesscan}. On the Google Speech dataset, \acrshort{fedlesscan} had a 25\% and 30\% improvement in experiment duration compared to \acrshort{fedavg} and \acrshort{fedprox} respectively.

% In the synthesized scenarios, we see the effect of stragglers on increasing round duration. In the scenarios with 10\% and 30\% straggler ratios, we notice that \acrshort{fedlesscan} maintains a lower duration across all experiments. When the percentage of stragglers surpasses a certain value, they must be invoked in almost all training rounds to meet the minimum number of clients per round. For instance, if a system has 100 clients and 50 are called every round, at least one straggler must be called every round if the straggler ratio exceeds 50\%; because the system contains less than 50 reliable clients, it has to choose from stragglers to complete the required number of clients per round. We notice this effect on \acrshort{fedlesscan} as the ratio of stragglers goes beyond a certain level. In the 50\% scenarios, we see a similar training time for all strategies except on the Google Speech dataset where \acrshort{fedlesscan} had an 18\% lower experiment duration. We justify this advantage by estimating the number of stragglers in the Speech experiment. The experiment was performed using 542 clients. At a 50\% straggler ratio, the number of reliable clients is about 272. Our approach is not bound to choose from stragglers each round because the number of participants per round is 200 (<272). On the other hand, at a 70\% straggler ratio, the system contains 162 reliable clients. Consequently, Stragglers have to be selected every round to reach the minimum number of clients (200). We see this in the 70\% scenarios, where all approaches have similar experiment times across all datasets. 


%%% cost

% To analyze the cost of the experiments, we had to estimate the cost of stragglers since stragglers can either miss their round or fail. Their running cost still factors in the experiment cost. The three approaches determine the round time by the slowest client participating in the current round or a specific timeout. In the worst-case scenario, stragglers can increase costs by wasting resources doing computations on wasted contributions. Therefore, we estimate the cost of stragglers as the cost of running the functions for the round duration. As we discussed in section~\ref{sec:metrics}, we use the computation model~\cite{gcf_cost} provided by Google Cloud to calculate the expected client cost. In this section, we examine the experiment costs and compare \acrshort{fedlesscan} to both \acrshort{fedavg} and \acrshort{fedprox}.


To analyze the cost of the experiments, we had to estimate the cost of stragglers since stragglers can either miss their round or fail. However, their running cost still factors into the experiment cost. In the worst-case scenario, stragglers can increase costs by wasting resources doing computations on wasted contributions. As a result,  we estimate the cost of stragglers as the cost of running the functions for the entire round duration. As described in \S\ref{sec:metrics}, we use the cost model for Google Cloud Functions~\cite{gcf_cost} for calculating the cost of the clients. 

Table~\ref{tab:cost-analysis} shows the cost for the different strategies, datasets, and scenarios. For the \textit{standard scenario} with MNIST, we observe a 6.8\% and 50\% cost reduction for our strategy as compared to \texttt{FedAvg} and \texttt{FedProx}. Similarly for the FEMNIST and Google Speech datasets in the \textit{standard scenario}, we observe cost reductions of about 2\%, 20\% and 12\%, 27\% as compared to \texttt{FedAvg} and \texttt{FedProx} respectively. On the other hand, for the Shakespeare dataset, \texttt{FedProx} performed better than our strategy and \texttt{FedAvg} by 4\% and 6\% respectively. We observe that the efficiency of our strategy becomes more visible as the number of stragglers in the system increases. For all the scenarios with a varying number of stragglers, our strategy has the minimum cost as compared to the other two strategies. For the \textit{straggler (\%) scenarios}, our strategy consistently achieved lower experiment cost across all datasets with an average cost reduction of 25\% and 32\% as compared to \texttt{FedAvg} and \texttt{FedProx} respectively.

% For the MNIST, FEMNIST, Shakespeare, and the Google Speech dataset we observe cost reductions of 19\%, 37\%, 18\%, 23\%, 20\%, and 30\%, 40\% with our strategy as compared to \texttt{FedAvg} and \texttt{FedProx} respectively.


% \todonils{Calculate average cost reduction in straggler scenarios wrt fedavg, and fedavg}

% Table~\ref{tab:cost-analysis} shows the cost of each experiment grouped by strategy and dataset. Investigating experiment cost for MNIST dataset shows that \acrshort{fedlesscan} has a 9\% lower cost than \acrshort{fedavg} and 40\% lower cost compared to \acrshort{fedprox} in standard scenario. We notice that the \acrshort{fedlesscan} efficiency becomes more visible as the number of stragglers in the system increases. In the synthesized scenarios, \acrshort{fedlesscan} maintains the cost advantage over \acrshort{fedavg} while \acrshort{fedprox} had the highest cost.

% For the FEMNIST dataset, \acrshort{fedlesscan} had the lowest overall experiment cost in all scenarios. Furthermore, \acrshort{fedprox} had the highest overall cost. In the standard scenario, \acrshort{fedlesscan} was more cost-efficient compared to \acrshort{fedavg} and \acrshort{fedprox} by 2.2\% and 20\% respectively.  In the synthesized scenarios, the average cost across all scenarios for our strategy was 18\% and 23\% lower compared to \acrshort{fedavg} and \acrshort{fedprox} respectively.  

% For the Shakespeare dataset, the same trend continues where \acrshort{fedlesscan} had a lower cost across all experiments. The cost gap among the three strategies was not significant in the standard scenario. Nevertheless, \acrshort{fedprox} performed better than \acrshort{fedlesscan} and \acrshort{fedavg} by about 4\% and 6\% respectively. In the synthesized scenarios, \acrshort{fedlesscan} achieve  an average experiment cost which was 20\% lower compared to \acrshort{fedprox} and \acrshort{fedavg}. Notice that we ran the experiment for a few rounds with fewer clients each round. As a result, the small scale of the experiment might underestimate the cost gains for \acrshort{fedlesscan}. 


% We further investigate the cost performance of our large-scale experiment using the Google Speech dataset.
% The Cost analysis results follow a trend similar to MNIST and FEMNIST datasets. \acrshort{fedlesscan} had the lowest cost compared to the other approaches across the five experiments. In standard settings,  \acrshort{fedlesscan} was 12\% more cost-efficient compared to  \acrshort{fedavg}. Moreover, \acrshort{fedlesscan} had 27\% lower cost than \acrshort{fedprox}. In the synthesized settings, The average cost gains across experiments increase to about 30\% when compared to \acrshort{fedavg} and 40\% when compared to \acrshort{fedprox}.


==> sections/system_design.tex <==
% In this section, we explain the enhancements added to the \acrshort{fedless} platform. These improvements aim to make the platform easier to use and provide the prerequisite architectural changes to include \acrshort{fedlesscan}.
In this section, we describe our extensions to the open-source system and framework \emph{FedLess}~\cite{fedless}. 

% These include the modifications to make \texttt{FedLess} more easier to use and the different system components required for implementing \texttt{FedLesScan}.


% With these modifications, we aim to make \texttt{FedLess} more easier to use and provide the required system components for implementing \texttt{FedLesScan}.

\subsection{Extensions to FedLess}
\label{sec:extfedless}
Figure~\ref{fig:arc-fedless} provides an overview of the modified system architecture of \emph{FedLess}~\cite{fedless}, with the different added system components highlighted in blue. 
The first significant enhancement is to the \emph{FedLess} controller. Previously, the controller required a complex deployment configuration and ran on a Kubernetes (K8s)~\cite{k8s} cluster with deployed OpenWhisk (OW)~\cite{openwhisk}. To overcome this, we completely removed the dependencies on  OW and K8s. To this end, the controller is now a lightweight process that can run on any system that includes its dependencies without any infrastructure management. A major challenge with distributed systems is the cost~\cite{jonas2017occupy}, ease of development, and debugging. Previously, the development and debugging of client/aggregation functions in \emph{FedLess} required their deployment on an actual FaaS platform (\S\ref{sec:faas}). To mitigate this, we implemented a mocking system in \emph{FedLess} that enables developers to run and debug the entire system on a single machine. We achieved this by adding different mock components to the controller that simulate the behavior of the actual components. It should be noted that using mock clients and aggregator does not require any additional effort from the user's side and everything is handled internally by the Mock \textit{Invoker}. The mocking system is activated by passing the \texttt{-mock} flag to the controller. Moreover, we abstracted the aggregation support to enable its implementation with any FaaS platform.

% In the previous version of \texttt{FedLess}, the aggregation of model updates was only possible with functions deployed on OW. To remove dependencies from a specific FaaS platform, we abstracted the aggregation support in \texttt{FedLess} to be usable with any FaaS platform.
% A major challenge in distributed systems is the ease of developem

To implement our strategy with \emph{FedLess}, we added a \textit{Strategy Manager} component to the controller. It is responsible for controlling the behavior of the selected strategy and contains two sub-components, i.e., the \textit{client selection} and the \textit{aggregation} scheme. The former is responsible for selecting the clients involved in a particular training round, while the latter is responsible for the type of aggregation algorithm used. Furthermore, to store the behavioral data of the clients, such as the number of failures, training duration, and the training rounds missed (\S\ref{sec:behavedata}), we added a client history collection to the database. The overall FL training workflow with our strategy remains similar to the one described in~\cite{fedless} with minor changes required for fetching/updating the behavioral data of clients.
% As the parameter server, \texttt{FedLess} uses MongoDB~\cite{mongodb}. 

%I think the training workflow will be explained in the algorithm

% It contains two sub-components, i.e., 

% \todomc{Aggregator specific components}
% \todomc{Stretegy specific components}
% \todomc{Write a small paragraph about training workflow, cannot include the figure}

% Figure~\ref{fig:arc-fedless} provides an overview of the modified system architecture and the core system components. 
% The first significant enhancement is in the \acrshort{fedless} controller. Previously, the \acrshort{fedless} controller ran in an Openwhisk cluster on top of a Kubernetes deployment. Therefore, even for debugging, getting started with the platform required a complex deployment configuration. One of the main objectives of a \acrshort{faas}-based \acrshort{fl} platform is its abstraction of the infrastructure management layer away from the developer. We addressed this limitation by removing the need for Openwhisk and Kubernetes. In the new architecture, \acrshort{fedless} controller runs on any machine that includes its dependencies without any infrastructure management. As a result, the cost and time needed for development and maintenance should decrease compared to the old architecture.

% We also added multiple sub-components in the \acrshort{fedless} controller. The strategy manager controls the behavior of the selected strategy. Each strategy contains the following:
% \begin{itemize}
% \item Client selection Scheme: Function responsible for clients selected for this training round.
% \item Aggregation Scheme: The aggregation scheme used by the aggregation function.
% \end{itemize}
% Developers can switch between different strategies with a single command line parameter. 

% Furthermore, \acrshort{fedless} used to support aggregation only on functions deployed in the local Openwhisk cluster. We abstracted the aggregation function to be usable on any self-hosted or public cloud provider. The effect of these changes lies in the ability to set up the platform quickly. The system no longer requires setting up the \acrshort{fedless} controller. Moreover, the system is no longer locked to using a specific serverless platform. On the database side, we added client history collection to store information about clients' behavior, such as failures, training duration, and the identifiers of missed rounds. We rely on the obtained behavioral data to implement our strategy and measure clients' performance. We also include components to facilitate debugging the platform. We explain their details in the next section.

% \subsubsection{System Debugging Capabilities}
%   \todonils{Does not seam relevant to the paper does it?}
% One of the main challenges in a distributed system is developing and debugging the whole system. Critically developers spend a considerable amount of time tuning the model's hyperparameters. Furthermore, debugging client functions is even more challenging, especially when the functions are deployed using cloud providers. Therefore, we introduced a mocking system in \acrshort{fedless} which enables developers to run and debug the whole platform on a single machine. The  \acrshort{fedless} controller contains mock components \textit{Mock Invoker}, \textit{Mock Client}, and \textit{Mock Aggregator} that simulates the behavior of the real component. The Mock Client is a Class that runs the same code present in the client functions. The Mock Aggregator is a Class that runs the aggregation process locally. When running the \acrshort{fedless} controller in debug mode, the Mock Invoker is activated and passed as a parameter to the Strategy Manager. After clients are selected to participate in the current round, the Strategy Manager delegates the clients' invocation to the Mock Invoker, which invokes multiple instances of the Mock Client class. When the clients finish training, the Mock Invoker receives a signal from the Strategy Manager to invoke the Mock Aggregator. The process repeats until the end of the training session. The developer can activate the mocking feature by specifying the \textit{--mock} parameter when running the \acrshort{fedless} controller.


% \subsection{Configuration and Training Workflow}

% % \begin{figure}[!htb]
% %   \centering
% %   \includegraphics[width=\linewidth]{figures/fedless_system/fedless_workflow_new.pdf}
% %   \caption{The training workflow of a typical training round in \acrshort{fedless} }\label{fig:fedless-flow}
% % \end{figure}

% Although the core idea of \acrshort{fedless} did not change, the training workflow changed slightly to accommodate the new architectural changes. Furthermore, the new flow should facilitate the implementation of other strategies, particularly \acrshort{fedlesscan}, with minimal communication costs. The communications required to invoke and authenticate clients remain the same.

%  Figure~\ref{fig:fedless-flow} demonstrates the communication among \acrshort{fedless} components in a typical training round.
% As we discussed in Section~\ref{sec:fedless-old}, the FL admin configures the model, dataset, and hyperparameters before starting the training. In the beginning, the controller fetches invocation tokens from the authentication server. Next, the controller fetches the clients' behavioral data from the \acrshort{fedless} database. Based on the selected strategy, a subset of the clients is chosen to participate in the current round. The controller invokes the client function using the invocation tokens. In the next step, the client function contacts the authentication server to validate the invocation token. Upon successful validation, the clients fetch the latest global model from the parameter server and perform the training locally while collecting information about the current training progress. When the training is complete, the clients upload the new local model to the parameter server and push the collected information to the client History collection. Next, the client function responds to the controller signaling the end of the training. At the end of the training round, the controller adjusts the participant's behavioral attributes based on the strategy and pushes them back to \acrshort{fedless} database. Afterward, the controller invokes the local aggregation function, which combines the clients' results into a new global model. At the end of the round, the controller invokes a subset of the clients for evaluation. The process then repeats for subsequent rounds.

==> tab/accuracy_analysis.tex <==
\begin{table}
\centering

\begin{adjustbox}{width=8.8cm,  center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multirow{3}{*}{\textbf{ Dataset}} & \multirow{3}{*}{\textbf{ Strategy}} & \multicolumn{10}{c|}{\textbf{Ratio of Stragglers}}                                                                                                                                          \\ 
\cline{3-12}
                                   &                                     & \multicolumn{2}{c|}{\textbf{Baseline}} & \multicolumn{2}{c|}{\textbf{10\%}} & \multicolumn{2}{c|}{\textbf{30\%}} & \multicolumn{2}{c|}{\textbf{50\%}} & \multicolumn{2}{c|}{\textbf{70\%}}  \\ 
\cline{3-12}
                                   &                                     & \textbf{Acc}   & \textbf{EUR}          & \textbf{Acc}   & \textbf{EUR}      & \textbf{Acc}   & \textbf{EUR}      & \textbf{Acc}   & \textbf{EUR}      & \textbf{Acc}   & \textbf{EUR}       \\ 
\hline
\multirow{3}{*}{MNIST}             & FedAvg                              & 0.981          & 0.99                  & \textbf{0.983} & 0.89              & \textbf{0.972} & 0.70               & 0.971          & 0.49              & 0.977          & 0.31               \\ 
\cline{2-12}
                                   & FedProx                             & 0.935          & 0.98                  & 0.972          & 0.88              & 0.960           & 0.69              & 0.962          & 0.49              & 0.967          & 0.29               \\ 
\cline{2-12}
                                   & FedLesScan                          & \textbf{0.985} & \textbf{0.99}         & 0.976          & \textbf{0.98}     & \textbf{0.972} & \textbf{0.96}     & \textbf{0.974} & \textbf{0.74}     & \textbf{0.979}  & \textbf{0.44}      \\ 
\hline
\multirow{3}{*}{FEMNIST}           & FedAvg                              & 0.756          & 0.99                  & 0.765          & 0.89              & 0.790           & 0.69              & 0.779         & 0.49              & 0.744           & 0.3                \\ 
\cline{2-12}
                                   & FedProx                             & 0.753          & 0.96                  & \textbf{0.778} & 0.80              & 0.756          & 0.64              & \textbf{0.785}  & 0.46              & 0.731           & 0.28               \\ 
\cline{2-12}
                                   & FedLesScan                          & \textbf{0.776} & \textbf{0.99}         & 0.770          & \textbf{0.97}     & \textbf{0.785} & \textbf{0.93}     & 0.774          & \textbf{0.80}      & \textbf{0.753} & \textbf{0.50}       \\ 
\hline
\multirow{3}{*}{Shakespeare}       & FedAvg                              & \textbf{0.434} & 0.87                  & \textbf{0.430}  & 0.80              & \textbf{0.401}   & 0.60               & 0.402   & 0.41              & 0.428           & 0.31               \\ 
\cline{2-12}
                                   & FedProx                             & 0.400          & 0.86                  & 0.399          & 0.78              & 0.396          & 0.58              & 0.345          & 0.40               & 0.38           & 0.29               \\ 
\cline{2-12}
                                   & FedLesScan                          & 0.388          & \textbf{0.94}         & 0.408          & \textbf{0.90}      & 0.400          & \textbf{0.86}     & \textbf{0.403}   & \textbf{0.72}     & \textbf{0.432}  & \textbf{0.53}      \\ 
\hline
\multirow{3}{*}{Google Speech}     & FedAvg                              & 0.766           & \textbf{0.99}        & 0.699            & 0.90               & 0.639           & 0.70               & 0.645           & 0.50               & 0.804           & 0.30                \\ 
\cline{2-12}
                                   & FedProx                             & 0.774          & \textbf{0.99}         & 0.664           & 0.89              & 0.709           & 0.70               & 0.694           & 0.49              & 0.759           & 0.29               \\ 
\cline{2-12}
                                   & FedLesScan                          & \textbf{0.794} & \textbf{0.99}         & \textbf{0.762}   & \textbf{0.97}     & \textbf{0.719}  & \textbf{0.90}      & \textbf{0.720}  & \textbf{0.86}     & \textbf{0.824}  & \textbf{0.74}      \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Accuracy and EUR values for the three strategies across different scenarios (\S\ref{sec:scenarios}) and datasets (\S\ref{sec:datasets}). The highlighted values represent the highest accuracy and EUR values for a particular dataset, strategy and scenario.}
\label{tab:acc-all}
\shrinkspace
\vspace{-1mm}
\end{table}


==> tab/cost_analysis.tex <==
% \usepackage{multirow}


\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{width=8.5cm,  center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{ Dataset}} & \multirow{2}{*}{\textbf{ Strategy}} & \multicolumn{5}{c|}{\textbf{Experiment Cost (\$)}}                                 \\ 
\cline{3-7}
                                   &                                     & \textbf{Standard} & \textbf{10\%} & \textbf{30\%} & \textbf{50\%} & \textbf{70\%}  \\ 
\hline
\multirow{3}{*}{MNIST}             & FedAvg                              & 2.90               & 3.90           & 6.00             & 8.00             & 10.40           \\ 
\cline{2-7}
                                   & FedProx                             & 5.50               & 6.40           & 7.60           & 9.21          & 11.03          \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{2.70}               & \textbf{3.86}           & \textbf{4.00}             & \textbf{5.99}             &\textbf{9.2}           \\ 
\hline
\multirow{3}{*}{FEMNIST}           & FedAvg                              & 13.50              & 16.19          & 17.87         & 20.54         & 24.70           \\ 
\cline{2-7}
                                   & FedProx                             & 16.67              & 17.29          & 19.40          & 22.42         & 25.80           \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{13.17}              & \textbf{14.58}         & \textbf{14.40}          & \textbf{14.81}         & \textbf{20.60}           \\ 
\hline
\multirow{3}{*}{Shakespeare}       & FedAvg                              & 5.40               & 6.60           & 9.21           & 12.50          & 15.40           \\ 
\cline{2-7}
                                   & FedProx                             & \textbf{5.12}              & 6.72          & 9.00             & 12.20          & 15.40           \\ 
\cline{2-7}
                                   & FedLesScan                          & 5.33              & \textbf{5.50}           & \textbf{6.75}          &\textbf{ 8.46}          & \textbf{12.00}             \\ 
\hline
\multirow{3}{*}{Google Speech}    & FedAvg                              & 1.98              & 3.90         & 6.40         & 8.30         & 10.50           \\ 
\cline{2-7}
                                   & FedProx                             & 2.39             & 4.60         & 6.77          & 8.70          & 10.80           \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{1.73}              & \textbf{2.70}         & \textbf{3.68}          & \textbf{4.20}          & \textbf{5.50}           \\
\hline
\end{tabular}
% }
\end{adjustbox}
\caption{Comparing training costs for the three strategies across different scenarios (\S\ref{sec:scenarios}) and datasets (\S\ref{sec:datasets}). The highlighted values represent the minimum experiment cost.}
\label{tab:cost-analysis}
\shrinkspace
\end{table}

==> tab/dataset_client_config.tex <==
\begin{table}[htp]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Benchmark} & \textbf{Dataset Name} & \textbf{No. of Clients} & \textbf{Clients Per Round} \\ \hline
-                  & MNIST                 & 300                     & 200                        \\ \hline
LEAF               & FEMNIST               & 300                     & 175                        \\ \hline
LEAF               & Shakespeare           & 100                     & 50                         \\ \hline
FedScale           & Speech Command        & 542                     & 200                        \\ \hline
\end{tabular}
}
\caption{Client configuration for each Dataset}
\label{tab:eval-clients}
\end{table}

==> tab/hyperparams.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{
\begin{adjustbox}{width=\columnwidth,  center}
\begin{tabular}{|c|ccc|cc|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Hyperparameters}}                                                           & \multicolumn{2}{c|}{\textbf{Number of Training Rounds}}                             \\ \cline{2-6} 
                                  & \multicolumn{1}{c|}{\textbf{Epochs}} & \multicolumn{1}{c|}{\textbf{Batch Size}} & \textbf{Learning Rate} & \multicolumn{1}{c|}{\textbf{Standard}} & \textbf{Straggler (\%)} \\ \hline
MNIST                             & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{10}                  & $1e-3$                 & \multicolumn{1}{c|}{60}                & 60                      \\ \hline
FEMNIST                           & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{10}                  & $1e-3$                  & \multicolumn{1}{c|}{40}                & 40                      \\ \hline
Shakespeare                       & \multicolumn{1}{c|}{1}               & \multicolumn{1}{c|}{32}                  & $0.8$                 & \multicolumn{1}{c|}{25}                & 25                      \\ \hline
Speech Command                    & \multicolumn{1}{c|}{5}               & \multicolumn{1}{c|}{5}                   & $1e-3$                  & \multicolumn{1}{c|}{35}                & 60                      \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Experiment hyperparameters for the different datasets (\S\ref{sec:datasets}) and experiment scenarios (\S\ref{sec:scenarios}).}

% The experiment was designed to enable the three strategies to reach similar range of accuracies in a specific number of rounds.
\shrinkspace
\label{tab:experiment-params}
\end{table}

==> tab/time_analysis.tex <==
% \usepackage{multirow}


\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{
\begin{adjustbox}{width=8.5cm,  center}
\begin{tabular}{|c|c|c|c|c|c|c|} 
\hline
\multirow{2}{*}{\textbf{ Dataset}} & \multirow{2}{*}{\textbf{ Strategy}} & \multicolumn{5}{c|}{\textbf{Experiment Time (mins)}}                               \\ 
\cline{3-7}
                                   &                                     & \textbf{Standard} & \textbf{10\%} & \textbf{30\%} & \textbf{50\%} & \textbf{70\%}  \\ 
\hline
\multirow{3}{*}{MNIST}             & FedAvg                              & 39.7              & 40.2          & 40.0            & \textbf{40.0}            & \textbf{40.0}             \\ 
\cline{2-7}
                                   & FedProx                             & 40.0                & 40.3          & 40.0          & \textbf{40.0}            & \textbf{40.0}             \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{23.7}              & \textbf{28.6}          & \textbf{27.3}          & \textbf{40.0}            & \textbf{40.0}             \\ 
\hline
\multirow{3}{*}{FEMNIST}           & FedAvg                              & 75.5              & 86.7          & 86.9          & \textbf{86.7}          & \textbf{86.7}          \\ 
\cline{2-7}
                                   & FedProx                             & 112.4               & 88.2            & 88.1            & 87.8            & 87.4             \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{70.9}              & \textbf{75.6}          & \textbf{82.8}          & 86.8          & \textbf{86.7}           \\ 
\hline
\multirow{3}{*}{Shakespeare}       & FedAvg                              & 217.0           & 217.0        & 217.0         & 216.9         & 216.8          \\ 
\cline{2-7}
                                   & FedProx                             & 217.0             & 217.0         & 217.0        & 217.0        & 216.7          \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{185.5}             &\textbf{ 215.5  }         & \textbf{205.2}           & \textbf{216.8}           & \textbf{216.6}            \\ 
\hline
\multirow{3}{*}{Google Speech}    & FedAvg                              & 20.3                & 40.1            & 40.1            & 40.0           & \textbf{40.0}             \\ 
\cline{2-7}
                                   & FedProx                             & 21.5              & 40.0           & 40.0           & 40.0           & \textbf{40.0}             \\ 
\cline{2-7}
                                   & FedLesScan                          & \textbf{15.1}                & \textbf{31.1}            & \textbf{28.8}            & \textbf{33.3}            & \textbf{40.0}             \\
\hline
\end{tabular}
% }
\end{adjustbox}
% \caption{total experiment time comparison between \acrshort{fedavg}, \acrshort{fedprox}, and \acrshort{fedlesscan} across all datasets. }
\caption{Comparing total time for the three strategies across different scenarios (\S\ref{sec:scenarios}) and datasets (\S\ref{sec:datasets}). The highlighted values represent the minimum training time for each experiment.}
\label{tab:total-time}
\shrinkspace

\end{table}
